A Lagrangian Relaxation for the Maximum Stable Set Problem

We propose a new integer programming formulation for the problem of finding a maximum stable set of a graph based on representatives of stable sets. In addition, we investigate exact solutions provided by a Lagrangian decomposition of this formulation in which only one constraint is relaxed. Some computational experiments were carried out with an effective multi-threaded implementation of our algorithm in a multi-core system, and their results are presented.

==> conclusion.tex <==
\section{Concluding remarks}
\label{sec:conclusion}

A decomposition for a new formulation for the SSP is proposed and
analyzed. An empirical comparison of this decomposition with the
standard formulation shows a significant improvement in the efficiency
of the branch-and-cut algorithm. According to experimental
observations, the standard formulation performs well with sparse
graphs. The decomposition leads to a better performance with denser
graphs. Additional gain in performance is attained with a parallel
implementation that explore the processing power of multicore systems.

As directions for further research, the effectiveness of the Lagrangian decomposition of the
representatives formulation (and its shared memory parallel implementation) for the SSP
makes this approach very promising for other problems involving stable
sets, like the vertex coloring problem and its generalizations.

